Revisit Micro-batch Clipping: Adaptive Data Pruning via Gradient Manipulation

Micro-batch clipping, a gradient clipping method, has recently shown potential in enhancing auto-speech recognition (ASR) model performance. However, the underlying mechanism behind this improvement remains mysterious, particularly the observation that only certain micro-batch sizes are beneficial. In this paper, we make the first attempt to explain this phenomenon. Inspired by recent data pruning research, we assume that specific training samples may impede model convergence during certain training phases. Under this assumption, the convergence analysis shows that micro-batch clipping can improve the convergence rate asymptotically at the cost of an additional constant bias that does not diminish with more training iterations. The bias is dependent on a few factors and can be minimized at specific micro-batch size, thereby elucidating the existence of the sweet-spot micro-batch size observed previously. We also verify the effectiveness of micro-batch clipping beyond speech models on vision and language models, and show promising performance gains in these domains. An exploration of potential limitations shows that micro-batch clipping is less effective when training data originates from multiple distinct domains.

==> intro.tex <==
\section{Introduction}
% 1.5 pages


\emph{Micro-batch clipping}~\cite{mcmahan2018general,ponomareva2023how} was initially introduced as a memory optimization technique for differentially private stochastic gradient descent (DP-SGD)~\cite{abadi2016deep}.
%
The method groups per-example gradients within a mini-batch into smaller micro-batches, clips the average gradient of each micro-batch, and updates the model with the mean of the clipped micro-batch gradients to avoid materializing all per-example gradients in memory.
%
Recent studies~\cite{wang2024unintended,wang2024efficiently} have surprisingly revealed that micro-batch clipping can enhance the performance of automatic speech recognition (ASR) models when used outside DP-SGD.
%
This finding has sparked interest in exploring micro-batch clipping as a standalone optimization technique, offering potential benefits in model performance.
%
However, the underlying mechanism driving this improvement remains poorly understood.

In this work, we aim to elucidate the behavior of micro-batch clipping through a combination of theoretical analysis and empirical evaluation.
%
Specifically, we conceptualize micro-batch clipping as a specialized form of data pruning~\cite{sorscher2022beyond}.
%
Unlike traditional data pruning techniques, which deterministically exclude redundant data, micro-batch clipping adaptively suppresses samples that hinder convergence, referred to as ``\emph{draggers}'', recognizing that a data sample's helpfulness can change throughout training.
%
Guided by this intuition, we introduce Assumption~\ref{aspt:dragger} to capture certain properties of the draggers' gradients, which are later empirically verified in Section~\ref{subsec:empirical_evidence_dragger}.
%
Based on the assumption, we analyze the convergence-to-stationary-points rate for both standard SGD and micro-batch clipping on smooth loss manifolds and summarize the results in in Table~\ref{tab:rate_summary}.
%
We can observe that the introduction of draggers slows down the convergence rate for SGD by a constant factor, while the usage of micro-batch clipping \emph{asymptotically accelerates the convergence rate}, at the cost of an additional constant bias term.
%
The bias term provides an explanation for the phenomenon observed in prior works~\cite{wang2024unintended,wang2024efficiently} where performance improvements are only seen with specific micro-batch sizes.
%
Concretely, because this term does not vanish with increasing iterations, the performance gain is contingent upon the magnitude of this term being sufficiently small.
%
According to Theorem~\ref{thm:mcsgd_main}, only certain micro-batch sizes minimize the bias term, thus explaining this effect.
%
% We hypothesize that only certain a decrease in $b$, the micro-batch size, leads to a stronger suppression of dragger gradients and increases the value of $c$.
% %
% Thus, the denominator of the constant term will be maximized at some certain micro-batch sizes.
% %
% The hypothesis that $c$ is decreasing with respect to $b$ is empirically validated in Section~\ref{subsec:empirical_evidence_c}.





\begin{table}[t]
  \caption{Convergence Rate}
  \label{tab:rate_summary}
  \centering
  \begin{tabular}{l|c|c|l}
    \toprule
     & Dragger & Clipping & Convergence Rate\\
    \midrule
    Thm 9~\cite{bu2024automatic} & \xmark & \xmark  & $\frac{1}{T^{1/4}}\sqrt{2L(\loss_0-\loss_*)+\frac{\sigma_b^2}{B}}$     \\
    Thm~\ref{thm:sgd_main} & \cmark & \xmark & $\frac{1}{T^{1/4}}\sqrt{\frac{4L}{(1-\epsilon)^2}(\loss_0-\loss_*) + \frac{2\sigma^2}{(1-\epsilon)B}}$       \\
    % Theorem 6 in~\cite{bu2024automatic} & \xmark & \cmark & $\min_{r\in(0, 1)}\frac{\sqrt{b}\sigma_b}{\sqrt{B}r} + \frac{4\sqrt{L(\loss_0-\loss_*)}}{\sqrt{T}\min_{c\in(0, 1)}f(c, r)}$ \\
    Thm~\ref{thm:mcsgd_main} & \cmark & \cmark  &  $\frac{\sigma}{(\sqrt{b}\epsilon-\sqrt{\epsilon(1-\epsilon)})\cdot(1+c)}+\frac{1}{\sqrt{T}}\cdot\mathcal{O}(\loss_0-\loss_*+\frac{1}{2L})$      \\
    \bottomrule
  \end{tabular}
\end{table}


% %
% Specifically, , introduced in this work, was verified.
% %
% Additionally, the inverse relationship between $c$ and $b$ was confirmed, supporting the explanation for the existence of an optimal micro-batch size between 1 and the mini-batch size.
%
% We also apply micro-batch clipping to train models for vision and language tasks to explore the border of micro-batch clipping's border of benefit.
% %
% It turns out that on single-task vision/language models, micro-batch clipping still provides substantial performance improvement.
% %
% However, when migrating to multi-task models, micro-batch clipping introduces trade-offs between different tasks due to the multimodal distribution of the gradients for different tasks.
%
To test the effectiveness of micro-batch clipping outside the speech domain, we apply it to vision and language models and observe promising performance improvements.
%
Another interesting observation is that micro-batch clipping's efficacy diminishes when facing multi-domain training data, particularly when data sizes between domains are unbalanced.
%
This may be attributed to the method hindering the convergence of domains with fewer samples by treating them as draggers.


